Total Recall: a Customized Continual Learning Method for Neural Semantic Parsers

This paper investigates continual learning for semantic parsing. In this setting, a neural semantic parser learns tasks sequentially without accessing full training data from previous tasks. Direct application of the SOTA continual learning algorithms to this problem fails to achieve comparable performance with re-training models with all seen tasks because they have not considered the special properties of structured outputs yielded by semantic parsers. Therefore, we propose TotalRecall, a continual learning method designed for neural semantic parsers from two aspects: i) a sampling method for memory replay that diversifies logical form templates and balances distributions of parse actions in a memory; ii) a two-stage training method that significantly improves generalization capability of the parsers across tasks. We conduct extensive experiments to study the research problems involved in continual semantic parsing and demonstrate that a neural semantic parser trained with TotalRecall achieves superior performance than the one trained directly with the SOTA continual learning algorithms and achieve a 3-6 times speedup compared to re-training from scratch. Code and datasets are available at: https://github.com/zhuang-li/cl_nsp.

==> analysis.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/stat_compare_origin.pdf}
    \caption{Stability of the base parser by using fine tuning.}
    \label{fig:overall_stability}

\end{figure}
We investigate catastrophic forgetting in details from the following two perspectives:
\begin{itemize}
    \item what kind of parse actions are easily forgotten when learning new tasks, and what kind of parse actions are unforgettable across tasks?
    \item How does our continual learning method help mitigate catastrophic forgetting?
\end{itemize}
We extend the empirical study~\cite{toneva2018empiricalStudyForgettable} in a standard classification setting for semantic parsing. Instead of conducting example-level analysis, we aggregate results to analyze parse actions in each of the three dataset respectively.

Given a previous task $\mathcal{T}^{(i-1)}$ and a current task $\mathcal{T}^{(i)}$, we consider an action from $\mathcal{T}^{(i)}$ as \textit{forgettable} for a model if its recall on a random sample in $\mathcal{T}^{(i-1)}$ decreases after learning $\mathcal{T}^{(i)}$, otherwise we call the action \textit{unforgettable}. For each dataset, we randomly select a permutation of the tasks $\{\mathcal{T}^{(1)}, ..., \mathcal{T}^{(K)}
\}$ and train our base parser sequentially. We compute the recall of each action on the \lqu{train/test?} set of the previous task $\mathcal{T}^{(i-1)}$ and the current task $\mathcal{T}^{(i)}$  after learning $\mathcal{T}^{(i)}$. The recalls are used to identify forgettable and unforgettable actions between $\mathcal{T}^{(i-1)}$ and $\mathcal{T}^{(i)}$.%In order to determine whether an action is forgettable by chance or not, we run a \lqu{which statistical test?} to check its accuracies significantly increases or decreases between adjunct tasks. Based on the test results, we group actions into forgettable and unforgettable for each dataset.

Among all actions, we differentiate also between cross-task actions and task-specific actions. %A cross-task action exists in each task, otherwise it is a task-specific one. 
Fig. \ref{} illustrates the proportions of forgettable and unforgettable actions grouped by cross-task and task-specific actions after learning a task $\mathcal{T}^{(i)}$ using standard fine-tuning, while Fig. \ref{} shows the statistics using our continual learning method. The figures about the other two datasets can be found in Appendix. \lqu{A grouped stacked bar plot, x-axis denotes different task, at each task i, you show two bars, one for cross task and another for task specific. Each stacked bar is divided by forgettable and unforgettable actions. One figure only for one dataset.} As we can see, XXX

To inspect to what degree actions are forgotten, we plot the amount of recall changes in the initial task after learning each new task via boxplots for cross-task and task-specific actions, respectively. \lqu{You plot grouped box plots, in each group, one for cross-task, another for task-specific, we measure accuracy change of task 1 w.r.t. each new task. You draw a figure for fine-tuning, and a figure for our method.} As illustrated in Fig. \ref{}, XXX

Catastrophic forgetting leads to instability of predictions across tasks. For a seen example, the parser may increase/decrease the rank of the gold action in its predictive distribution at time $t$. We collected the ranks of gold actions for each example in the seen tasks after learning a new task. We ran \lqu{XXX} test to compute p-values regarding rank changes. The lower the p-values, the more frequent the ranks change. From Fig. \ref{fig:overall_stability} we can see that the \overnight corpus is definitely the most difficult one, followed by \nlpmapq and \nlpmapc. \lqu{Add the one for continual learning as well} Our continual learning method can improve stability on all three datasets. A close inspection on forgettable and unforgettable actions regarding stability (Appendix) shows that XXX \lqu{a bit strange results}.  

%We define an example $\bm{x}_i$ from the task $\mathcal{T}^{k}$ as forgettable w.r.t. an action $a_j$ if the model can correctly predict the action $a_j$ derived from its LF while learning the task $\mathcal{T}^{k}$ but fails to estimate the action correctly after learning a new task. Let $\bm{a}^* = \arg\max_{\bm{a}} p(\bm{a} | \bm{x}_i)$ and $\bar{\bm{a}}$ denote its ground-truth action sequence, we use a binary variable $\text{accu}^{\mathcal{T}^{k'}}_i \mathds{1}_{a^*_j = \bar{a}_j}$ to indicate whether the example correctly predicts the action $a_j$ on $\bm{x}_i$ after learning a task $\mathcal{T}^{k'}$. Given a pair of tasks $\mathcal{T}^{a}$ and $\mathcal{T}^{b}$, for each action $a_j$ in $\mathcal{T}^{a}$, we count the number of forgettable examples w.r.t. $a_j$ for \lqu{XX} number of 




==> tab-bert-fix.tex <==
\begin{table}[ht]
\centering
  \resizebox{0.95\textwidth}{!}{%
  \begin{tabular}{|c|c c|c c|cc|}
    \toprule
    \multirow{2}{*}{Methods} &
      \multicolumn{2}{c|}{\overnight} &
      \multicolumn{2}{c|}{\nlmapq} &
      \multicolumn{2}{c|}{\nlmapc} \\
      & W  & A & W  & A & W  & A \\
      \midrule
    Fine-tune & 12.46 & 11.76 &  46.21  & 41.61  & 45.51  & 44.09 \\
        \hline
    \ewc & 17.03 & 18.54 & 48.99 & 46.05  & 10.51 & 9.12 \\
    \emr & 39.02 & 39.93 & 45.52& 40.90 & 55.53 &54.29 \\
    \aemrt & 39.82 & 44.76 & 52.44 &47.61  & 52.15  & 50.33 \\
    \hline
    \oracle (All Tasks) & 64.70 & 63.90 & 73.20 & 71.91 &69.80 & 67.57 \\
    \bottomrule
  \end{tabular}%
  }
    \caption{LF Exact Match Accuracy (\%) of parsers using BERT as the embedding layer and with its parameters fixed.}
  \label{tab:bert-fix}
    \vspace{-2mm}
\end{table}

==> tab-sample_back.tex <==
\begin{table*}[ht]
\centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c|cccccc|cccccc|cccccc|}
    \toprule
    \multirow{3}{*}{Methods} &
      \multicolumn{6}{c|}{\overnight} &
      \multicolumn{6}{c|}{\nlmapc} &
      \multicolumn{6}{c|}{\nlmapq} \\
    &\multicolumn{2}{c}{10} &
      \multicolumn{2}{c}{25} &
      \multicolumn{2}{c|}{50} & 
      \multicolumn{2}{c}{10} &
      \multicolumn{2}{c}{25} &
      \multicolumn{2}{c|}{50} & 
      \multicolumn{2}{c}{10} &
      \multicolumn{2}{c}{25} &
      \multicolumn{2}{c|}{50}\\
    
      & W  & A  & W  & A & W  & A & W  & A & W  & A & W  & A & W  & A & W  & A & W  & A \\
      \midrule
    \random & 38.57 & 40.45 & 59.28& 57.56 & 45.29 & 46.01 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41  \\
    \fss & 29.85 & 30.89 & 38.72 & 40.30 & 94.51 & 83.41 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 \\
    \gss & 45.29 & 46.01 & 58.36 & 56.95 & 80.79 &76.64 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 \\
    \prior & 22.31  & 24.84 & 30.29 &34.19  & 38.65 & 43.00  & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 \\
    \balance & 28.46 & 30.40 & 37.39 & 39.23 & 42.93 &44.24 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 \\
    \hline
    \lfs & 29.51 & 31.04 & 38.44 & 39.48 & 47.05 & 47.96 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 \\
    Ours & 28.64 & 30.70 & 40.05  & 42.00 & 46.49 & 48.36 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41 & 38.57 & 40.45 & 59.28& 57.56 & 94.51 & 83.41\\
    \bottomrule
  \end{tabular}%
  }
    \caption{Accuracy (\%) of \emr with different sampling strategies and buffer sizes 10, 25 and 50}
  \label{tab:sample}
    \vspace{-2mm}
\end{table*}
